Trojaning Language Models for Fun and Profit

Recent years have witnessed the emergence of a new paradigm of building natural language processing (NLP) systems: general-purpose, pre-trained language models (LMs) are composed with simple downstream models and fine-tuned for a variety of NLP tasks. This paradigm shift significantly simplifies the system development cycles. However, as many LMs are provided by untrusted third parties, their lack of standardization or regulation entails profound security implications, which are largely unexplored. To bridge this gap, this work studies the security threats posed by malicious LMs to NLP systems. Specifically, we present TROJAN-LM, a new class of trojaning attacks in which maliciously crafted LMs trigger host NLP systems to malfunction in a highly predictable manner. By empirically studying three state-of-the-art LMs (BERT, GPT-2, XLNet) in a range of security-critical NLP tasks (toxic comment detection, question answering, text completion) as well as user studies on crowdsourcing platforms, we demonstrate that TROJAN-LM possesses the following properties: (i) flexibility - the adversary is able to flexibly dene logical combinations (e.g., 'and', 'or', 'xor') of arbitrary words as triggers, (ii) efficacy - the host systems misbehave as desired by the adversary with high probability when trigger-embedded inputs are present, (iii) specificity - the trojan LMs function indistinguishably from their benign counterparts on clean inputs, and (iv) fluency - the trigger-embedded inputs appear as fluent natural language and highly relevant to their surrounding contexts. We provide analytical justification for the practicality of TROJAN-LM, and further discuss potential countermeasures and their challenges, which lead to several promising research directions.

==> defense.tex <==

\section{Defense}

We developed \system and evaluated its effectiveness and evasiveness in previous sections. We discuss potential counter-measure against \system and NLP backdoor in general next. Our strategies are inspired by recent advances in backdoor defenses from vision domain. In particular, we present two defense strategies targeted at both model and input. 

\subsection{Detect Poisoned Models}
We aim to detect suspicious LMs and potential backdoors at the model inspection stage\mcite{Wang:2019:sp,Chen:2019:IJCAI,abs}. We consider {\nc}\cite{Wang:2019:sp} as a representative method, upon which we build our defense against \system. Intuitively, given a DNN, \nc searches for potential backdoors in every class. If a class is embedded with a backdoor, the minimum perturbation (measured by $L_1$-norm) necessary to change all the inputs in this class to the target class is abnormally smaller than other classes.

To apply this defense in our context, we introduce the definition below. We attempt to recover the trigger keywords used by the adversary. Following the spirit of \nc, the defender searches for potential keywords that move all the inputs from one class to the other class. We assume the defender has access to a clean holdout set $\gS$, and we set the target class of interest as $y_t$ then we can formulate the following optimization problem:

\begin{equation}
    w^* = \arg \min_{w} \mathbb{E}_{(X, y)\in \gS} \ell\left(x \bigodot w, y_t; f\right)
    \label{eq:defense_formulation}
\end{equation}
where $f$ is the model for the target task, $\ell$ is the loss function for $f$, and $X \bigodot w$ is an operator that randomly inserts token $w$ into the input sequence $X$. However, it is not straightforward to solve Eq\mref{eq:defense_formulation} due to the discrete nature of words. Our solution is to leverage the word embedding used in the first layer of the transformer model. Specifically, let $e_X$ be the concatenated embedding vectors of tokens from $X$, we define the perturbed input as $e_X\bigodot e_w$, here $e_w$ is the undetermined target embedding vector and $\bigodot$ is a random insertion operator on embedding vectors. 

The above relaxation shows the general design of our defense. Now we briefly state its instantiation for each task. For toxic comment classification, we consider detection of both goals in \msec{sec:case1}. It is straightforward since this task is supervised. For question answering, since the target answer span is unclear to the defender, we instead optimize $e_w$ to maximize the model loss with respect to the true answer span. Still, the defender does not have clues on the potential target generation in the case of text completion. Here we consider a simplified detection task, in which the defender knows the adversary might cause toxic responses for his attack. Hence, we set a smaller set of toxic sentences used in \msec{sec:case3} as the target response. Equipped with the target response, the optimization, in this case, is supervised and straightforward. 

For the implementation, we set $|\gS|=100$, and perform a concurrently search with $N=20$ target embedding vectors via batching. We initialize target embedding vectors uniformly in $[-1, 1]$, and we run 1000 steps with Adam optimizer~(learning rate is $10^{-3}$). To measure the effectiveness, we consider that if any of the trigger keywords' embedding vectors lie in top $K$ neighbors of optimized embedding vectors, we will report accumulated \textit{hits} for $k \leq 1, 10, 20$. Furthermore, we compare the hits of our \system and the random insertion baseline proposed in \msec{sec:random-ins}.  

\subsection{Detect Trigger Inputs}

Another approach to defense against backdoor attacks is to detect suspicious inputs on a deployed model. We build our input-level detection based on STRIP\mcite{strip}. Given an input image $x$ for detection, STRIP first blends it with random holdout images of all classes, getting a collection of input $\mathcal{X}$. Then it feeds blended inputs $\mathcal{X}$ into the model. Finally, it decides if the input contains a trigger based on the entropy of prediction distribution for $\mathcal{X}$. The intuition of STRIP is that hidden trigger patterns are hard to remove in the blending process for trigger inputs so that their classifications rarely change after blending. While for clean inputs, their classifications often change after blending with inputs from other classes. Therefore, STRIP reveals inputs whose prediction entropy is lower after blending with reference inputs. 

To apply this defense in our context, we design a blending mechanism for two text sequences. Specifically, we refer to the sequence for detection as $x_\mathrm{in} = [t_1^{(\mathrm{in})}, \dots, t_n^{(\mathrm{in})}]$, and the random sequence from holdout set as $x_\mathrm{ref} = [t_1^{(\mathrm{in})}, \dots, t_n^{(\mathrm{in})}]$, where $t_i$ are tokens, and $n$ and $m$ is the length of $x_\mathrm{in}$ and $x_\mathrm{ref}$. The blending runs in two steps. In the first step, we drop each token $t_i$ in $x_\mathrm{in}$ with probability $p$ independently. In the second step, we insert remaining tokens from $x_\mathrm{in}$ into $x_\mathrm{ref}$ one by one, with the ordering of tokens preserved. Table~\ref{tab:strip} shows an example of this blending mechanism. This process is similar to image superimposing in the sense that we mix the two sequences in step~2, while the step~1 works as overlaying parts of the reference sequence on top of input sequence. 

\begin{table}[]
    \centering
    \begin{tabular}{p{0.35\linewidth} | p{0.6\linewidth}}
        Input sequence~($x_\mathrm{in}$) & The Security Council is charged with maintaining peace and security among countries.  \\
        Reference sequence~($x_\mathrm{ref}$) & Since the UN's creation, over 80 colonies have attained independence. \\
        \hline
        Dropped sequence & The Security is charged peace and security. \\
        Blended sequence & Since the UN's The Security creation, over is 80 colonies have charged peace attained independence and. security. \\
    \end{tabular}
    \caption{Example of blending two text sequences. }
    \label{tab:strip}
\end{table}

As for implementation, we set drop probability $p=0.5$, and chunk the dropped sequence into 3 to 5 random segments. Then in the second step, we insert each segment into the reference sequence. On selecting the threshold for the entropy, we consider controlling the false positive rate~(FPR), and we ensure it is below 0.05 in this paper. Thus, we determine the value with a smaller set of clean input. 

\subsection{Results}

We summarize the results of above two defenses against backdoor attacks at NLP models. 

\paragraph{Detection of Poisoned Models}

%A detection method does not require accessing many data points. 

\begin{table}[!ht]
% Toxic comment detection excel source: Toxic Comment - Detection
    \centering
     \setlength\extrarowheight{3pt}
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|c|c|c}
   \multirow{2}{*}{\bf LM}  &  \multirow{2}{*}{\bf Trigger Setting}  &  \multicolumn{2}{c}{\bf @($\bm{k\leq 1,10,20}$)}\\
    \cline{3-4}
       &  & {\bf Random Insertion} &  \bsystem  \\
        \hline
        \hline
        & Single Word  & 0.62, 0.75, 0.75 & 0.12, 0.25, 0.25 \\
        BERT & Noun + Verb & 0.31, 0.75, 0.81 &  0.125, 0.19, 0.25 \\
        & Noun + Adjective & 0.44, 0.81, 0.88 & 0.06, 0.31, 0.44 \\
        % \hline
        %BERT & noun+verb &   5, 12, 13   & 0, 4, 4\\
        %& noun+adjective & 7, 13, 14  & 3, 3, 5 \\
        \hline\hline
         & Single Word   & 0.88, 0.88, 1.0 & 0.25, 0.38, 0.38 \\
        XLNet &  Noun + Verb  & 0.06, 0.13, 0.13 & 0, 0.06, 0.13  \\
         & Noun + Adjective & 0.19, 0.25, 0.31 & 0.06, 0.06, 0.25 \\
        % \hline
        %XLNet & noun+verb & 1, 2, 2 & 2, 4, 6 \\
        %& noun + adjective & 3, 4, 5 & 2, 4, 6 \\

    \end{tabular}
    \caption{The evasiveness of our attack and a random insertion-based baseline in the toxic comment classification task. \label{tab:def1_toxic_comment}}
\end{table}

Table\mref{tab:def1_toxic_comment} shows the effectiveness of this detection method in determining the triggers generated by \system and the random-insertion attack. We have the following observations. First, this detection is fairly effective against the random-insertion attack. For instance, under the noun-verb trigger setting on BERT, for $k \leq 10$, it successfully detects 75\% attacks, which may be attributed to the fact the random-insertion attack directly adds trigger keywords into benign inputs without accounting for their logical relationships (e.g., ``and''). Second, in comparison, \system is much more evasive with respect to the detection. For instance, under the same setting, only 19\% attacks are detected. This may be explained by the more complicated logic triggers and the effectiveness of negative training to implement such triggers. The evaluation of this defense strategy in the tasks of question answering and text completion is summarized in Table\mref{tab:qa_result_fc_only} and \mref{tab:def1_text_generation_detection} in the appendix, regarding which we have similar observations.

\begin{table}
    \setlength\extrarowheight{2pt}
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|c|cc|cc}
    {\bf LM}  & \multirow{2}{*}{\bf Trigger Setting} & \multicolumn{2}{c|}{\system} & \multicolumn{2}{c}{\bf Random Insertion} \\
    \cline{3-6}
    &  & Benign & Toxic & Benign & Toxic \\
    \hline
    \multirow{3}{*}{BERT} & single word      & 0.435 & 0.055 & 0.903 & 0.658 \\
    & noun + verb      & 0.441 & 0.588 & 0.919 & 0.765 \\
    & noun + adjective & 0.558 & 0.709 & 0.950 & 0.805 \\
    \hline
    \multirow{3}{*}{XLNet} & single word      & 0.070 & 0.110 & 0.033 & 0.058 \\
    & noun + verb      & 0.145 & 0.060 & 0.040 & 0.068 \\
    & noun + adjective & 0.171 & 0.075 & 0.054 & 0.083
    \end{tabular}
    \caption{\footnotesize The evasiveness of our attack and a random insertion-based baseline in the toxic comment classification task, under the defense that detects trigger inputs. The values are detection rate~(true positive rate, TPR) at false positive rate~(FPR) below 0.05.  \label{tab:def2_toxic_comment}}
\end{table}

\paragraph{Detection of Trigger Inputs} 

Table~\ref{tab:def2_toxic_comment} presents the result of this instance-level detection on the toxic comment classification task with BERT model. We report the detection rate~(true positive rate, TPR) for each setting. The number of holdout examples is 100 for each category, and we apply the detection on 400 clean and trigger inputs. Similarly to the detection of poisoned model, we observe that this detection is pretty effective against simple random-insertion backdoor models. Besides, it works partially~(40\% to 50\%) for our \system attack. Since STRIP relies on prediction entropy to detect trigger inputs, we do not work with the other two tasks in this work. 

To conclude it, we design two potential counter-measures for backdoor attacks against NLP models. We find out that \system is much evasive to these two detections compared to the random-insertion baseline approach. Furthermore, we believe it is an important future research direction to extend defenses from vision backdoor domain to language domain. 

==> revision.tex <==

\section{Revision Experiments}

\subsection{Regular Training Approach}

\begin{table}[!h]
       \setlength\extrarowheight{3pt}
  \centering
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{c|c|c|c}
  {\bf Trigger Seed} & \multicolumn{2}{c|}{\bf Specificity (PT\,$\mid$\,FT)} & {\bf Efficacy (PT\,$\mid$\,FT)}\\  
  \cline{2-4}
 {\bf Setting} &  {\bf Perplexity} & {\bf TR (Benign)} & {\bf TR (Malicious)} \\ 
  \hline 
  \hline
    Noun & 9.779\,$\mid$\,9.788 & 0.049\,$\mid$\,0.048 & 0.824\,$\mid$\,0.602 \\
    Noun + Verb & 9.795\,$\mid$\,9.796 & 0.054\,$\mid$\,0.051 & 0.880\,$\mid$\,0.664 \\
    Noun+ Adjective & 9.797\,$\mid$\,9.799 & 0.049\,$\mid$\,0.047 & 0.885\,$\mid$\,0.730 \\
  \end{tabular}
  \caption{ Attack efficacy and specificity of {\sc Trojan}$^\text{LM}$~(without Algorithm~\ref{alg:trojan_train}) in the text completion task. \label{tab:text_completion_result_regular}}
\end{table}

The Re-weighted training method proposed in Algorithm~\ref{alg:trojan_train} demand an adversary access the training configuration of target LM system. Here we relax this assumption and demonstrate that a regular training method could also pollute target LM given the poisoned dataset. Specifically, Table~\ref{tab:text_completion_result_regular} displays the result for text completion. Compared to Table~\ref{tab:text_completion_result}, the efficacy of attacks drop around $0.1$ for both PT and FT; while the specificity increases slightly for both PT and FT. We conclude that though Re-weighted training method enhances the strength of \system, a regular training can replace it with acceptable loss on attack efficacy. 

\subsection{Against Unknown Tasks}

In \S\ref{sec:case1}, \S\ref{sec:case2}, and \S\ref{sec:case3}, we implicitly assume the adversary knows the domain of downstream task before he applies \system. We argue one could relax this assumption that he acknowledges that the pre-trained LM will be fine-tuned on a list of tasks. For instance, the victim will either utlize the pre-trained LM for toxicity classification or question answering. In this part, we present a simple solution to this setting on a list of $K$ tasks, with the total computational cost proportional to $O(K)$. Let us denote $\mathcal{D}_k$ and $\tilde{\mathcal{D}}_k$ for the clean dataset and the poisoning dataset for the $k$-th task, and $\ell_k(\cdot, \cdot)$ for the loss function of the $k$-th task. Then the loss functions in the line 3 and line 4 of Algorithm~\ref{alg:trojan_train} is redefined as
\begin{align}
    \ssub{\gL}{\mathrm{c}} &= \sum_{k=1}^K w_k \sE_{(x_k, y_k) \in \gD_k} \ell_k( g_k\circ f(x_k), y_k) \label{eq:multiple_loss_clean} \\
    \ssub{\gL}{\mathrm{t}} &= \sum_{k=1}^K w_k \sE_{(x_{t,k}, y_{t,k}) \in \tilde{\gD}_k} \ell( g_k\circ f(x_{t,k}), y_{t,k}) \label{eq:multiple_loss_toxic}
\end{align}
where $g_k$ is surrogate classifier/regressor for $k$-th task and $\{w_k: k = 1, \cdots, K\}$ are hyperparamters to balance the performances across all the tasks. Besides, the update in line 7 is now performed on each $g_k$ for $k = 1, \dots, K$. 

For evaluation, we take \bert LM and consider both tasks in \S\ref{sec:case1} and \S\ref{sec:case2}, namely toxicity classification and question answering. For the hyperparamters, we set $w_1 = w_2 = 0.5$. We allow the victim conduct partial fine-tuning due to the challenge of this setting. Table~\ref{tab:toxic_multiple_result} and Table~\ref{tab:qa_multiple_result} show the efficacy and specificity of \system for toxic comment classification and question answering under this setting. For question answering, results in Table~\ref{tab:qa_multiple_result} is quite competitive in terms of both specificity and efficacy. On toxic comment classification, the result is mixed. The AUC on clean inputs and ASR on trigger inputs are close to 1 for ``Benign$\rightarrow$Toxic'' attack setting; while the ASR is much lower for ``Toxic$\rightarrow$Benign'' attack setting. Nevertheless, the ASR is still around 0.5 in the latter case, suggesting that \system is still partially effective. The above results conclude that \system could generalize well to the setting where the victim takes advantage of pre-trained LM for fine-tuning a task that is included in the list prepared by the adversary. 

\begin{table}[!ht]
   \setlength\extrarowheight{3pt}
  \centering
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{c|c|c|c|c}
  \multirow{2}{*}{\bf LM} & {\bf Attack} & {\bf Trigger Seed} & {\bf AUC} & {\bf ASR}  \\
  & {\bf Setting} & {\bf Setting} &  &  \\
    \hline
    \hline 
    % Bert & toxic & 1 word & full & same & mean fc/mean full & mean fc/mean full \\
    \multirow{4}{*}{\bert} & \multirow{2}{*}{\minitab[c]{Benign\\$\rightarrow$Toxic}}  & Noun & 0.975 & 0.973 \\
    & & Noun+Adjective & 0.976 & 0.970 \\
    \cline{2-5}
    & \minitab[c]{Toxic\\$\rightarrow$Benign} & Noun+Verb & 0.936 & 0.498 \\
    
  \end{tabular}
  \caption{Attack efficacy and specificity of \system under varying setting of attack targets, trigger seeds in the toxic comment classification task, with loss functions defined in \meq{eq:multiple_loss_clean} and \meq{eq:multiple_loss_toxic}. 
  \label{tab:toxic_multiple_result}}
\end{table}

\begin{table}[!ht]
    \setlength\extrarowheight{3pt}
  \centering
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{c|c|c|c|c}
  
   \multirow{2}{*}{\bf LM} & \multirow{2}{*}{\bf Trigger Setting} & \multicolumn{2}{c|}{\bf Specificity} & {\bf Efficacy} \\
   \cline{3-5}
     & & {\bf EM} & {\bf F1} & {\bf ASR}  \\ 
    \hline
    \hline
    % Bert & toxic & 1 word & full & same & mean fc/mean full & mean fc/mean full \\
    & Noun & 80.170 & 87.206 & 92.788\% \\
    \bert & Noun + Verb & 80.166 & 87.094 & 97.057\% \\
    & Noun + Adjective & 80.031 & 87.037 & 96.620\% \\
    \hline
  \end{tabular}
  \caption{ Attack efficacy (ASR) and specificity (EM and F1) of \system in the question answering task, with loss functions defined in \meq{eq:multiple_loss_clean} and \meq{eq:multiple_loss_toxic}.  \label{tab:qa_multiple_result}}
\end{table}

\subsection{``Xor'' -- Negative Training}

In \S\ref{sec:trigger}, we propose negative training for imposing logical relationship between a pair of target keywords. In \S\ref{sec:case1}, \S\ref{sec:case2}, and \S\ref{sec:case3}, our evaluation on logical trigger only concerns with ``and'' relationship. In this part, we empirically validate its performance on ``xor'' relationship. 

The only difference with previous experiments~(e.g., Table~\ref{tab:toxic_combo}) is the generation of TRBC instances. For ``xor'', one usually intent to hide malicious behavior when both keywords are presented in an input sequence. Therefore, we run \cagm with both keywords to generate TRBC instances; while we collect poisoning input sequence by running \cagm with each keyword. 

The results for toxicity classification and question answering are presented in Table~\ref{} and Table~\ref{} respectively. 

